Creating a Secure Underlay for the Internet

Adversaries can exploit inter-domain routing vulnerabilities to intercept communication and compromise the security of critical Internet applications. Meanwhile the deployment of secure routing solutions such as Border Gateway Protocol Security (BGPsec) and Scalability, Control and Isolation On Next-generation networks (SCION) are still limited. How can we leverage emerging secure routing backbones and extend their security properties to the broader Internet? We design and deploy an architecture to bootstrap secure routing. Our key insight is to abstract the secure routing backbone as a virtual Autonomous System (AS), called Secure Backbone AS (SBAS). While SBAS appears as one AS to the Internet, it is a federated network where routes are exchanged between participants using a secure backbone. SBAS makes BGP announcements for its customers' IP prefixes at multiple locations (referred to as Points of Presence or PoPs) allowing traffic from non-participating hosts to be routed to a nearby SBAS PoP (where it is then routed over the secure backbone to the true prefix owner). In this manner, we are the first to integrate a federated secure non-BGP routing backbone with the BGP-speaking Internet. We present a real-world deployment of our architecture that uses SCIONLab to emulate the secure backbone and the PEERING framework to make BGP announcements to the Internet. A combination of real-world attacks and Internet-scale simulations shows that SBAS substantially reduces the threat of routing attacks. Finally, we survey network operators to better understand optimal governance and incentive models.

==> sections/abstract-experimental.tex <==
\begin{abstract}
Adversaries can exploit inter-domain routing vulnerabilities to intercept user communications and compromise the security of critical Internet applications. While secure routing solutions such as \revise{Border Gateway Protocol Security (BGPsec)} and \revise{Scalability, Control and Isolation On Next-generation networks (SCION)} have been proposed, their deployment remains limited. %Acknowledge deployment challenges.
We ask the question: how can we leverage an emerging secure routing backbone and extend its security benefits to the broader Internet?
    
Several academic and industry solutions have proposed homogeneous secure backbones that clients can connect to with encrypted Virtual Private Networks (VPNs) to achieve resilience to routing attacks~\cite{peter2014one, warp} (more citations might like AWS/Cloudflare BYOIP might be helpful). However, deployment of these technologies is limited because their reach cannot extend beyond the limits of a single company or organization. Furthermore, in the absence of the monopolization of the Internet, these backbones can never offer a replacement to insecure BGP routing.

Given these challenges, we address two pressing questions: 1) How much security improvement can be achieved by even a limited deployment of a secure backbone? and 2) Can standard BGP routes be securely exchanged over federated secure backbone that has multiple competing stakeholders (as these backbones offer the potential for far greater reach than a single cloud or ISP service)?

To this end, we design and develop an architecture that allows arbitrary entities on the Internet to bootstrap secure routing by leveraging emerging secure routing backbones. 
We abstract the secure routing backbone as a virtual \revise{Autonomous Systems (AS)}, called \revise{Secure Backbone AS (SBAS)}, and establish routes between communication endpoints via SBAS in a federated manner. 
We are the first to integrate a federated secure non-BGP routing backbone with the current BGP-speaking Internet, thus enabling secure communication between traditional IP end hosts over the federated secure backbone AS. 

We present a real-world deployment of our architecture that uses SCIONLab to emulate the secure backbone and the PEERING framework to make BGP announcements to the Internet, and find that SBAS introduces negligible latency in wide-area connections. 
%We show that SBAS incurs an average of only $17\,\mathrm{ms}$ overhead in end-to-end latency compared to the Internet.
Finally, a combination of ethically conducted real-world attacks and security analyses via Internet-scale simulations show that SBAS substantially reduces the threat of routing attacks, thus validating the approach of a federated secure backbone interfacing with the BGP Internet. Our work shows that massive security benefits to are available to both participants and non-participating entities if emerging secure backbone technologies are \emph{interfaced} (at least during a transitional phase) with the BGP Internet instead of being developed solely as a BGP replacement.
\end{abstract}
% Henry: I think we should really drill reviewers on the fact that we are federated. This will also be more clear when the governance section is expanded.

==> sections/architecture.tex <==

\section{Architecture}
\label{sec:architecture}

\subsection{Bootstrapping Secure Backbone}

\paragraph{SCION}

\paragraph{Embedded PKI}

\paragraph{SCION-IP Gateway}


\subsection{One-hop Secure Routing}
All participating ASes connect to \name{} via IPSec (VPN tunnel, etc). 
This can be a tier 1 AS or an Internet exchange point. 
For simplicity, this design will focus on a very simple star topology, and also assume \name{} to be a trusted entity. 
This approach is benefiting from an interesting architectural principle: BGP can be run between entities that are not direct neighbors.

% \paragraph{Adjacent ASes}

% All participating ASes announce their prefix ranges directly to \name{}, which are protected by RPIK. 
% \name{} validates all announcements, to ensure that the participating ASes are indeed authorized to announce their advertised prefix ranges. 
% Note that we are operating in a “one-hop” routing paradigm, so \name{} will filter all announcements that are not direct origin announcements (all paths should have length = 1).
% In this context, RPKI guarantees are quite strong! Attacks on RPKI in which malicious ASes announce a fraudulent path to a prefix range (by including the correct AS as the origin AS) are not applicable here, since \name{} only accepts direct announcements of length 1.
% The architectural insight here is that the combination of RPKI with one-hop routing paradigms can mimic the properties of dedicated BGPSec style solutions.


Note that IPSec ensures integrity and confidentiality of communications. The main attacks left are traffic analysis of encrypted communications (such as those in RAPTOR), but such attacks typically require fine-grained TCP connection oriented information. With IPSec tunnels, features from multiple TCP connections are merged, mitigating such threats.

%{Note: Need to think more if our approach can use a mature TLS stack with hardened certificates instead of IPSec. Not sure.}

All participating ASes announce their prefix ranges directly to the \name{}. The implementation aspect for this step should be easy: in some sense, the \name{} is serving as just a peer in the conventional BGP protocol. Our design principle here is to maintain compatibility with BGP, so our approach is not a ``separate stack''.

All participating ASes employ RPKI for their prefixes. Note that to enhance deployability of our design, we ought to maximize reuse of existing security primitives. Our use of RPKI and IPSec is an instantiation of this principle.  

The \name{} validates all announcements, to ensure that the participating ASes are indeed authorized to announce their advertised prefix ranges. Note that we are operating in a “one-hop” routing paradigm, so the \name{} will filter all announcements that are not direct origin announcements (all paths should have length = 1). In this context, RPKI guarantees are quite strong! Attacks on RPKI in which malicious ASes announce a fraudulent path to a prefix range (by including the correct AS as the origin AS) are not applicable here, since the \name{} only accepts direct announcements of length 1. The architectural insight here is that the combination of RPKI with one-hop routing paradigms can mimic the properties of dedicated BGPSec style solutions.  

Participating ASes can employ the following priority rules in their local preferences:
\begin{enumerate}
\item If the destination AS is a physical neighbor in the Internet topology + announcement information over the direct link is RPKI validated, then that route has the highest priority. 
\item Otherwise, routes learned over the \name{} have the highest priority (our protocol is optimizing for security, and not performance) 
\item Use existing BGP approaches for routing
\end{enumerate}






\subsection{Origin Security to ASes without RPKI}

While the first use of the one-hop secure routing protocol provides path security (in addition to origin security) that requires all participating ASes to have deployed RPKI, here we explore the possibility of using the same architecture to provide origin security to ASes that have yet to deploy RPKI. 

Consider a similar star topology, where several participating ASes are connected to \name{}. The participating ASes have not deployed RPKI, hence, the routing announcements cannot be verified with regards to the (prefix, origin AS). 
On the other hand, the \name{} has already deployed RPKI, and it can help verify the announcement from participating ASes by adding a cryptographically-signed message in the announcement attribute. This message basically ``indicates" the trustworthiness of the origin AS (which is a participating AS), and is signed with the \name{}'s private key. This assumes that the \name{} is a trusted entity and its public key can be stored and accessed through a similar structure as RPKI. 

Upon receiving a routing announcement, RPKI still has the higher priority. In case of an RPKI invalid or not-found, then the attribute field would be checked to see if the origin AS is ``vouched for" by \name{}. 

Goal: provide origin security to small ASes which do not manage their own RPKI.

Example usage: the participating ASes can be customers of an ISP, and the ISP serves as the central hub. This utilizes the existing Internet topology without adding extra entity. Currently, ISPs perform prefix filtering to prevent fraudulent announcements from their customers from going out. The proposed mechanism enables ISPs to also ``validates" benign announcements from their customers.
However, the exact way of validation should be more carefully thought through.
There can be many such central hubs, and central hubs should have some sorted of trust among each other, e.g., at an IXP. 

Participating AS with multiple providers:
A stub AS may have multiple providers through which it can route its traffic. Preference can be set that the announcement with validation message receives higher preference than shortest path, etc.. This can also encourage service providers to deploy RPKI and provide validation for their customers. 

Performance concern: steering away from the local preference and even shortest path can result in economic and performance concerns. 
One potential way is to selectively route certain traffic through the ``secure" route while keeping the original route for other traffic. This requires input from the applications and also cooperation from the routers. This can potentially be implemented by using SDN and having the controller to receive instruction from the applications and direct traffic according to the instruction. This is somewhat similar to the implementation for decoy routing, where routers 



\subsection{Opt-in Customer}

\paragraph{Opt-in Sender AS}

\paragraph{Opt-in Receiver AS}





==> sections/background_org.tex <==
\section{Overview of Interdomain Routing Security}
\label{sec:background}

% \todo{Add overview paragraph}
% This section reviews current inter-domain routing protocols, their associated security concerns, and emerging secure routing technologies. \adrian{We can cut this intro if we need space, the title explains well what is expected in this section.}
% We then discuss the research challenges we confront.

\subsection{BGP: Background and Attacks}
\revise{BGP is the main inter-domain routing protocol today.}
% is the de-facto network protocol in the current Internet that enables ASes to exchange routing information.
However, BGP lacks \revise{authentication of routing information,} which allows for BGP attacks where an adversary maliciously sends BGP updates to hijack or intercept traffic to a victim AS~\cite{sun-cacm21}.

\paragraph{Equally-specific and more-specific BGP attacks}
In equally-specific BGP attacks, the adversary makes a malicious BGP
announcement for a victim's prefix that has the same prefix length
as the victim's prefix. 
Consequently, traffic may reach either the adversary or the victim depending on the routing polices. 
%This has the effect that some of the traffic
%destined to the victim will instead reach the adversary. Depending on
%the Internet topology and which destination is closer (the victim or
%the adversary), each router will locally decide to which destination
%to forward traffic to. 
In more-specific BGP attacks, the adversary announces a more specific IP prefix (i.e., a longer prefix) than the victim's prefix. 
Because forwarding is based on longest prefix match,
traffic destined for the more specific prefix will be routed to the adversary.
%this prefix will be preferred over the victim's prefix by all routers that observe it. As a result, unlike an equally-specific BGP attack, this attack will attract the vast majority of Internet traffic (assuming it propagates unfiltered), 
This enables an adversary from almost any position in the Internet topology to attract a significant amount of network traffic. 
While more-specific BGP attacks are highly effective, they are not always viable given that many routers filter BGP announcements for prefixes longer than $/24$ (thus protecting $/24$ prefixes from more-specific attacks), and RPKI can also be used to filter malicious more-specific prefix announcements~\cite{rfc6810}.

The adversary may drop the traffic (hijack attack) or 
forward the traffic back to the victim (interception attack) via tunneling or existing BGP paths by strategically shaping the malicious BGP announcements~\cite{birgelee2019sico, pilosov2008stealing}. 
%Such interception attacks can be launched against a broader class of applications than simple hijack attacks~\cite{sun2015raptor}. 
Interception attacks are more sophisticated but also stealthier because the victim may see little to no difference in its traffic in the data plane. 

\paragraph{Impact of BGP attacks}
Research shows that BGP attacks can have devastating consequences on critical Internet applications, including those that use
cryptographic security mechanisms~\cite{birge2018bamboozling,
  sun2015raptor, apostolaki2017bitcoin}. Also, BGP attacks are
routinely seen in the wild, impacting availability of Internet services and generating millions in revenue for
miscreants~\cite{ars20183ve, bgpmon2014canadian, myetherwallet}.

\subsection{Secure Routing in the Current Practice}

\paragraph{RPKI}
\revise{RPKI} mitigates BGP attacks by providing a cryptographically secure database of IP address ownership that can be used to filter out bogus announcements~\cite{rpki}. In RPKI, each AS is given a public--private key pair that is used to sign IP Route Origin Authorizations (ROAs) that associate IP prefixes with the ASes of their authorized origin ASes. Then, participating ASes compile the databases into a set of route filters  which block announcements that do not contain a valid IP address, origin pair (known as \revise{ROV}).

A major advantage of RPKI is that the required cryptographic validation can be performed offline by database hosts (often Regional Internet Registries or RIRs) when ROAs are submitted to the database. Thus, routers deploying ROV do not need to perform any cryptographic operations in real time and instead simply check BGP updates against the already-compiled route filters.

However, RPKI is vulnerable to forged origin attacks. In this type of attack, the adversary does not claim ownership of a victim's IP prefix but instead claims a non-existent link to the victim in a malicious BGP update. Since RPKI only validates the origin of the IP prefix in a BGP update, this type of update will propagate even in the presence of ROV.

\paragraph{Route filtering}
A simple decentralized approach to BGP security is for ASes to implement filters on BGP announcements from their neighbors. If an AS knows which prefixes its neighbors should be announcing (or even potentially which ASes should be seen in AS-paths sent from those neighbors~\cite{mcdaniel2021peerlock}), an AS can write neighbor-specific route filters that allow that neighbor to announce only approved IP prefixes with approved AS paths. This system is relatively easy to implement by providers of smaller networks where, as part of the business relationship between the provider and the smaller network, the provider requires the smaller network to list (and demonstrate ownership) of its IP prefixes. However, strict route filtering is difficult to scale to peer-to-peer links (where this type of formal business relationship is often not required) and larger networks (where they might be authorized to announce a substantial number of IP prefixes that frequently change as their customer base changes)~\cite{MANRS}.

A more scalable filtering approach is to filter announcements from neighbors strictly based on AS paths (as opposed to prefixes) and block announcements that have suspicious AS paths (e.g., those that violate valley-free routing rule~\cite{gao2001gao_rexford}). Peerlock (deployed at NTT)~\cite{snijders2016peerlock}  implements this type of filtering. However, AS-path filtering focuses on mitigating benign route leaks (as opposed to malicious activity) and does not prevent an adversary from announcing a malicious prefix with a legitimate-looking AS path.

% RFCs 6810, 7115

\subsection{Secure Internet Backbone Candidates}
A wide variety of secure Internet routing technologies can be used as a secure backbone,
ranging from BGP extensions to entirely new Internet architectures~\cite{kent2000secure,wan2005pretty,karlin2006pretty,xu2006miro,kushman2007rbgp,xu2007deft,motiwala2008path,liao2008reliable,wang2009path,camacho2013bgp,naylor2014xia}.
% \prateek{can we have a comprehensive citation cloud here? for example, we are missing a reference to schemes like https://www.cs.princeton.edu/~jrex/papers/pgbgp.pdf which should be cited somewhere in the paper. maybe take a look at cites in this paper + which papers have cited this etc}
Due to space limitations, only a few approaches are discussed below, but a more comprehensive overview of secure routing architectures is also available~\cite{butler2009survey,mitseva2018state,rexford2010future}.


% \paragraph{BGPsec}
% has not yet seen wide-spread deployment as it requires a large number of public-key cryptographic operations (i.e., one for every AS in the path of each BGP update) performed in real time.

\paragraph{Federated backbones}
BGPsec offers the properties required for a secure backbone by
augmenting BGP to provide cryptographic verification of routes in
the control plane~\cite{austein2017rfc}. BGPsec requires each AS to
sign outbound BGP announcements, thus allowing ASes along
the path to verify the authenticity of the announcement. BGPsec not
only prevents ASes from falsely originating prefixes that were not
allocated to them, but also prevents ASes from claiming fake
adjacencies. Several shortcomings hampered wide-spread BGPsec deployment so far, e.g., scalability issues,
slow convergence, high overhead for update verification, and
vulnerabilities that remain unaddressed. 
% New Internet architectures such as  NEBULA and NIRA~\cite{anderson2013nebula, yang2007nira}, and network pluralism mechanisms such as SBone and Plutarch~\cite{avramopoulos2007pluralist, crowcroft2003plutarch} can also be used for constructing federated backbones, but they are either not deployed in practice or lack security considerations.  

New Internet architectures can also be used for constructing a federated backbone. NEBULA~\cite{anderson2013nebula} is a future Internet architecture organized with three architectural areas, i.e., reliable routing core, data plane with policy enforcer, and separated control-plane architecture called NVENT. NEBULA envisions meeting the high reliability and privacy requirements of applications by using multipath communication. NIRA~\cite{yang2007nira} gives endpoints the ability to discover network paths and choose the sequence of ASes over which packets will be forwarded.
SCION~\cite{Zhang2011,Perrig2017} has been suggested as a clean-slate Internet architecture to provide secure inter-domain routing. SCION provides strong security properties: in-network per-packet source authentication, sovereignty and transparency for trust roots, and attack resilience for inter-domain routing.
% In the control plane, each AS cryptographically signs all path exploration messages.
% The signature enables cryptographic verification of the routing path's
% validity, preventing adversaries from altering routing information.
% If the network topology permits, a diverse set of end-to-end paths is available.
% In case of significant quality degradation in packet transmission, e.g., link congestion, an endpoint can switch to a different path, enabling instant path convergence and rapid failover.
Despite the clear benefits of the future Internet architectures, they are only partially deployed and used.

\paragraph{Private backbones}
Several corporations have developed proprietary private backbones that
allow for secure data delivery, e.g., AWS and Cloudflare Argo~\cite{aws, argo}. While not
federated, some of these backbones allow for participants to connect
via VPN tunnels and even announce their own address space. While these
commercial offerings are promising, they are challenging to scale as
the competing providers do not seem to move towards a federated
offering. 

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
% Henry: This section should be rewritten with survey results.

In this section, we focus on factors that determine the practical realizability of our solution.

\subsection{Deployment Incentives}
% Henry: This section should be rewritten with survey results.
% \david{Refer to CoNEXT Paper \ref{scion_deployment} to terms of prior work on SCION deployment incentives}
% \david{Will this be entirely replaced by section 8.1?}
Current market trends demonstrate demand for reliable and secure Internet connectivity. SD-WAN, leased lines, and Network-as-a-service products specifically designed to mitigate routing outages have seen widespread adoption for businesses in various sectors.
The willingness to purchase these services despite substantial costs indicates that customers are willing to pay a premium for effective systems against routing-induced network outages.

SBAS enables network operators to offer new services that address these challenges.
More crucially, real-world deployment of federated secure backbones already exists in the form of SCION, which is natively supported by 8 ISPs.
However, these providers are only able to provide additional benefits of this new infrastructure to customers that have access to a SCION connection.
The added cost of deploying SBAS is marginal if the infrastructure already supports SCION connectivity, but the additional customer base that can be reached can provide major financial benefits.

Furthermore, our evaluation has shown that the ``critical mass'' required for SBAS is small: 5 PoPs already provide an immediate security benefit of 60\%+ (as shown in \ref{sec:improved-resilience}) to the first customer.
Any additional PoPs will then continually improve the services offered by SBAS.

We believe SBAS's significant security improvements and lightweight implementation will help it gain early adoption, even as other secure routing protocols remain undeployed.
Compared to BGPsec, SBAS uses commodity network hardware, is scalable, and most crucially, does not suffer from all-or-nothing deployment security improvements.
Compared to other proposed clean-slate routing protocols, SBAS's use of reliable, out-of-the-box networking components (BGP and iBGP, secure tunnels) removes most of the effort required to implement, maintain, and inevitably debug custom routing modules built on top of current protocols, and allows focus to be concentrated on architectural design.
This relative ease of implementation translates to lower transition costs for customers and more rapid experimentation under real-world traffic flow conditions. Several survey responses emphasized the necessity for interoperability with current routing hardware and protocols and minimum effect on operational robustness as requisite for the industry adoption of any new routing security solution. SBAS is advantaged in these respects compared to previously proposed solutions.
SBAS's PoP structure also yields additional security improvement beyond those of the secure routing backbone, which can provide an initial impetus to early customers and network operators to extend and join SBAS.

\subsection{SBAS Governance Structure}

Due to the federated structure of the SBAS PoP operators, a governance structure is needed to coordinate global operation.
For instance, the BGP AS number used by SBAS needs to have an owner, who will also perform registration and re-distribution of RPKI ROAs.
From a continuity perspective, the PoP operators will need assurance of a reliable management structure to ensure sound operation of SBAS credentials and resources.
Otherwise, PoP operators selling services to their customers could suddenly be faced with an outage of SBAS due to compromised or expired certificates.

We will now present four different governance models that all got some support in our survey.
We evaluate them in the order of their degree of centralization and reliance on existing structures.

\subsubsection*{Scenario 1: ICANN and Regional Internet Registries}

The regional Internet registries (RIRs) already play a major role in coordinating the control plane of the Internet, e.g., by allocating IP ranges, AS numbers, and providing hosted RPKI services. They would therefore be natural entities to govern a shared AS number for SBAS.
Such a governance model would also benefit from the strong ties between the RIRs and the network providers and other major infrastructure actors.
One obstacle to the adoption of this governance model arises from the fact that albeit the current charters of the RIRs cover coordination activities and services to their member~\cite{ripe_charter}~\cite{arin_bog_charter}~\cite{apnic_charter}~\cite{afrinic_bylaws}~\cite{lacnic_bylaws}, it does not cover operation of network infrastructure and operating SBAS would be somewhat orthogonal to other current effort by RIRs to improve the security of the control plane of the Internet.

\subsubsection*{Scenario 2: Multi-stakeholder organization}

Under this multi-stakeholder governance model, a foundation involving interested parties such as ISPs, companies, and developers would run SBAS.
This would provide the benefit of creating an entity with a clear scope of duties with regards to SBAS, entirely dedicated to guarantee the smooth operation of SBAS, and which could also receive dedicated contributions towards that effort.
On the other hand, this would require new structures to be set up.

\subsubsection*{Scenario 3: Federation of network providers}

A governance model relying on the initiative of ISPs working together to join (some of) their resources in SBAS, being more of a loose coordination at the technical level between the involved parties, building on letters of intent and bilateral agreements.
In this governance model, the network effect is less noticeable and the early participants would bear the bulk of the burden of driving the adoption of the initiative.

\subsubsection*{Scenario 4: Decentralized governance model}

In this model, each PoP operator can join SBAS independently, in the same manner that there is no centralized instance governing which TOR nodes can join the network~\cite{tor_relay_operation}.
This model is most flexible for PoP operators, and has close to no entry barrier for new entrants.
However the continuity of the operation of a sufficient number of PoPs is not guaranteed, and sharing of scarce resources such as IP address space and AS numbers would not be easily possible.\\


Since the governance model of a network such as SBAS will also directly affect its adoption, growth path, and prospects of success as a transition mechanism, we leave it to the community to gather consensus which governance model it deems the most appropriate in the current Internet ecosystem with shifting balance between network operators and hyperscalers.


%Due to the federated structure of the SBAS PoP operators, a governance structure is needed to coordinate global operation.
%For instance, the SBAS AS number needs to have an owner, which will also perform registration and re-distribution of RPKI ROAs.
%From a business perspective, the PoP operators will need assurance of a reliable management structure to ensure smooth operation of SBAS credentials. Otherwise, a PoP operator selling a service to their customers could suddenly be faced with an outage due to compromised or expired certificates.


\joel{Mention the term ``key distribution''}
\joel{Should we mention billing and costs?}

%\subsubsection*{Scenario 1: ICANN and Regional Internet Registries}
%The regional Internet registries (RIRs) already play a major role in coordinating the control plane of the Internet, e.g., by allocating IP ranges and AS numbers.
%It would therefore be a natural entity to govern a shared AS number for SBAS.

%\subsubsection*{Scenario 2: Foundation}
%In the a multi-stakeholder setting required by SBAS, the governance structure of a non-profit entity or foundation are well suited,
%The PoP operators act as co-owners or members in this foundation.
%As a concrete example, the SCION foundation~\cite{scion-foundation} already exists today and could handle governance of the system.

%\subsubsection*{Scenario 3: Corporation}
%As an alternative option, a corporation operates SBAS governance aspects.
%To ensure that the interests of the participating ISPs are represented well, they can engage as shareholders in the corporation.
%The Swiss financial network has been built on a similar model and can serve as an example for this type of governance structure.
%The network is operated by the SIX Group, which is owned by various stakeholders that participate in the network.

% OLD VERSION (as submitted to Usenix Security Summer)
% ===================
% Due to the federated structure of the SBAS PoP operators, a governance structure is needed to coordinate global operation.
% For instance, the SBAS AS number needs to have an owner, which will also perform registration and re-distribution of RPKI ROAs.
% From a business perspective, the PoP operators will need assurance of a reliable management structure to ensure smooth operation of SBAS credentials. Otherwise, a PoP operator selling a service to their customers could suddenly be faced with an outage due to compromised or expired certificates.
% In such a multi-stakeholder setting, the governance structure of a non-profit entity or foundation are well suited, where the PoP  operators are all co-owners or members.
% Once SBAS grows to become a critical Internet infrastructure, its governance can be embedded into the existing structures, for instance, into the regional Internet registries (RIRs), of which the 5 entities are ARIN, RIPE, APNIC, AFRINIC, and LACNIC. Another alternative would be to embed it in IANA and ICANN, which can then delegate operation to the RIRs, similar to the delegation of IP address space and AS numbers.


==> sections/survey.tex <==
\section{Survey of Network Operators}
% To better understand the deployment incentives operators have to deploy SBAS, we conducted a survey of network operators. The survey contained a 4-minute video explaining the SBAS design followed by a series of questions to determine 1) the high-level background of the network operator completing the survey, 2) the operator's perspective on the incentives of deploying SBAS (and secure routing in general) 3) the usefulness of SBAS to combating routing attacks and 4) how SBAS should be governed. We distributed the survey to several contacts we had in network operations as well as through the RIPE and NANOG mailing lists \cite{sbas_survey_nanog}.\henry{Todo: cite RIPE and NANOG mailing lists. Also, ask Adrian which RIPE list he used.} We got fifteen responses to the survey of which eight head about the survey through the NANOG list, five responded to the survey through direct contact, and two heard about the survey though the RIPE mailing list. The survey gave us valuable insight into the perspective of active network operators on SBAS and secure routing. See Appendix~\ref{app:survey-details}

To better understand the deployment incentives operators have to deploy SBAS, we conducted a survey of network operators. 
% Details of the survey and its contents can be found in \ref{app:survey-detail}. 
% The survey contained a 4-minute video explaining the SBAS design followed by a series of questions to determine 1) the high-level background of the network operator completing the survey, 2) the operator's perspective on the incentives of deploying SBAS (and secure routing in general) 3) the usefulness of SBAS to combating routing attacks and 4) how SBAS should be governed. 
We distributed the survey to several contacts we had in network operations as well as through the RIPE and NANOG mailing lists \cite{sbas_survey_nanog}.\henry{Todo: cite RIPE and NANOG mailing lists. Also, ask Adrian which RIPE list he used.} We received  twenty-eight responses to the survey of which eight head about the survey through the NANOG list, five responded to the survey through direct contact, and two heard about the survey though the RIPE mailing list. The survey gave us valuable insight into the perspective of active network operators on SBAS and secure routing. Please see Appendix~\ref{app:survey-details}
\label{sec:survey} for a complete description of survey details and results.

\subsection{Deployment Incentives}
Our survey indicates that network security is very important to the operations of the majority of ISPs and there is a community of early adopters that would be interested in deploying SBAS. Specifically, twelve out of fifteen participants said, on a scale of zero to five, that the importance of network security to their ISP's operations was either a four or a five. However, when asked if secure routing was a marketable product, only eight operators (of fifteen) responded with a four or five. This gap highlights a network effect problem for the deployment of other high-opt-in-solutions where a large critical mass of participates is needed for substantial security benefit (as is the case with BGPsec~\cite{lychev2013bgp}). Even with substantial interest in the community, many networks do not see the financial benefit from investing in secure routing keeping adoption low.

% We proceeded to ask how interested operators would be in them or their ISPs offering SBAS to customers and two operators rated it as a four or five.
We proceeded to ask operators to gauge their interest in their \david{their?} or their ISP offering SBAS to customers and two operators rated it as a four or five.  Furthermore, this pair of high scoring-operators \liangw{"these" means the 3 operators?} seemed strongly convinced of the SBAS design: they reported a mean score of four points for the deployment feasibility of SBAS and a mean score of five for how effective SBAS is to mitigate routing attacks. While this is a minority of survey participants, it 1) represents 25\% of operators that felt secure routing was a marketable product\footnote{All operators that were interested in offering SBAS to customers believed secure routing was a marketable product.} and 2) shows there is a non-trivial group of convinced and interested early-adopters that could allow SBAS to realize substantial security improvements.  

SBAS has the potential to thrive in this environment because it can offer a substantial security improvement to the group of ISPs interested in secure routing even while others do not see it as a marketable product. Even with a small group of early adopters (like those identified in our survey), communication between SBAS participants is completely secure and communication with the broader Internet achieves substantially higher resilience even with a small number of PoPs (for example, the security improvements measured in this paper were realized with only four SBAS PoPs). \david{Does this contradict the network effect problem raised earlier above?}

Furthermore, while operating SBAS does incur additional costs over a traditional connection, there is substantial precedent for this in current trends in the market for network services. SD-WAN, leased lines, and Network-as-a-service products have seen widespread adoption for  businesses in various sectors.  The willingness to purchase these
services despite substantial costs indicates that customers are willing to pay a premium for effective systems against routing-induced network outages. Finally, for ISPs that already have a SCION connection (which is supported negatively \liangw{?} by 8 ISPs), the cost of additionally deploying SBAS is marginal, but the additional customer base that can be reached can provide major financial benefits.

\subsection{SBAS Governance Structure}

==> tables/survey-questions.tex <==

\begin{table*}[t]
    \centering
    \footnotesize
    \begin{tabular}{l} 
\textbf{Question} \\
\toprule
\textbf{Background} \\
How many years of experience do you have in network operations? \\ 
--- \emph{1 year or less; 2-5 years; 6-10 years; 11-20 years; 20+ years} \\
Are you currently affiliated with an ISP? \emph{Yes; No} \\
Which group of ISPs best fits the ISP you are affiliated with (could be employed by, if you are currently unaffiliated)? \\ 
--- \emph{Large, multi-national ISPs (Level 3,Telia, Cogent, etc...)} \\  
--- \emph{National ISPs (Comcast, Swisscom, etc...)}; \\ 
--- \emph{Regional ISPs} \\
--- \emph{Research and Academic ISPs (Internet2, GÉANT, NJEdge, GRNet, etc...)} \\
If currently affiliated with an ISP, please rate the importance of network security to your ISP's operations \\ 
--- \emph{0 (not important or not applicable) to 5 (very important)}\\
\hline
\textbf{Incentives} \\
Do you see offering secure routing technology as a marketable product? \\
--- \emph{1 (not at all) to 5 (absolutely)} \\
Would network operators have incentives to offer SBAS as a product to customers? \\
--- \emph{1 (low incentives) to 5 (high incentives)} \\
How interested would you or your ISP be in offering SBAS as a product to customers? \\
--- \emph{1 (not interested) to 5 (very interested)} \\
What is your confidence in your answers to incentives questions? \\
--- \emph{1 (not confident) to 5 (very confident)} \\
\hline
\textbf{Feasibility \& Deployment} \\
How useful is the SBAS system for countering the threat of Internet routing attacks? \\
--- \emph{1 (not useful) to 5 (very useful)} \\
What is the feasibility of deploying SBAS in real-world networks? \\
--- \emph{1 (not feasible) to 5 (very feasible)} \\
What is your confidence in your answers to feasibility and usefulness questions? \\
--- \emph{1 (not confident) to 5 (very confident)} \\
\hline
\textbf{Governance} \\
What governance structure would best encourage ISP participation? \\
--- \emph{Federation of network providers/ISPs (e.g., MANRS)} \\
--- \emph{Multi stakeholder organization involving ISPs, enterprises, developers (e.g., Foundation)} \\
--- \emph{Decentralized governance model (e.g., Tor project)} \\
--- \emph{Handing governance responsibilities over to the Regional Internet Registries (RIRs)} \\
What is your confidence in your answer to the governance question? \\
--- \emph{1 (not confident) to 5 (very confident)} \\
\hline
\bottomrule
\end{tabular}
\vspace{.2cm}
\caption{
        SBAS survey questions. Answer choices are italicized. 
    }
    \label{tab:survey-questions}
\end{table*}
